Design Considerations for 3RRR Parallel Robots with Lightweight, Approximate Static-Balancing

Balancing parallel robots throughout their workspace while avoiding the use of balancing masses and respecting design practicality constraints is difficult. Medical robots demand such compact and lightweight designs. This paper considers the difficult task of achieving optimal approximate balancing of a parallel robot throughout a desired task-based dexterous workspace using balancing springs only. While it is possible to achieve perfect balancing in a path, only approximate balancing may be achieved without the addition of balancing masses. Design considerations for optimal robot base placement and the effects of placement of torsional balancing springs are presented. Using a modal representation for the balancing torque requirements, we use recent results on the design of wire-wrapped cam mechanisms to achieve balancing throughout a task-based workspace. A simulation study shows that robot base placement can have a detrimental effect on the attainability of a practical design solution for static balancing. We also show that optimal balancing using torsional springs is best achieved when all springs are at the actuated joints and that the wire-wrapped cam design can significantly improve the performance of static balancing. The methodology presented in this paper provides practical design solutions that yield simple, lightweight and compact designs suitable for medical applications where such traits are paramount.

==> content/Acknowledgment.tex <==

% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...


==> content/Appendices.tex <==

% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%

\appendix{

\begin{algorithm}[htbp] \nonumber
 \caption{Nonlinear LS Minimization}
 \label{algo:cal_1:LS}
 %
 \begin{algorithmic}[1]
 \footnotesize
 \Require $TargetPoses(q,\Phi,\Psi)$ \Comment {Data set for minimization process}

 \State \textbf{START} Initialize: $\mb{\vec{x}}$,\hspace{2mm} $M_i \gets 100$ \Comment {Minimization parameters vector}

 \While{$M>\epsilon_{\tau} \hspace{2mm}and \hspace{2mm}iter_{i}<iter_{max}$}

     \State $\vec{\bs{\Gamma}}(\vec{x}) = \left[\bs{\Gamma}_{11}; \bs{\Gamma}_{21};...;\bs{\Gamma}_{3N}\right]$, \hspace{2mm}
          \hspace{2mm} \hspace{4mm} \Comment {Aggregated torque vector}  \Comment {N number of Target Poses}

     \State $\bigtriangleup\bs{\Gamma} = \frac{\partial\bs{\Gamma}}{\partial\vec{x}}\bigtriangleup\vec{x}$,\hspace{2mm} $\frac{\partial\bs{\Gamma}}{\partial\vec{x}} = \bs{J}_A$, \hspace{2mm} \\
     \State $\bs{J}_A = \begin{bmatrix}\frac{\partial\bs{\Gamma}_1}{\partial\vec{x}} \\ \frac{\partial\bs{\Gamma}_2}{\partial\vec{x}} \\ \vdots \\ \frac{\partial\bs{\Gamma}_{3N}}{\partial\vec{x}}\end{bmatrix}$ \Comment {Gradient of cost function}

     \State Update $\mb{\vec{x}}_{i+1}$:
     \begin{align}
       &\mb{\vec{x}}_{i+1} = \mb{\vec{x}}_i - \eta \mb{J}_A^{\boldsymbol{+}}\vec{\Gamma} \\
           %\label{eqn:algo:NLS_update_k}
       &M_i = \frac{\vec{\bs{\Gamma}}^T\vec{\bs{\Gamma}}}{2N}
          %\label{eqn:algo:J_M_plus}
    \end{align} \Comment {$\eta$ step-size matrix}
 \EndWhile
\State $\mb{\vec{x}}^{*} \gets \mb{\vec{x}}_i$
 \Ensure ${\mb{\vec{x}}^{*}}$
\end{algorithmic}
\end{algorithm} } 

==> content/wire_cam_kinematics.tex <==
\subsection{Wire Cam Kinematics}


\par Satisfying the conditions for a balanced system can be achieved by having the total potential energy of a mechanism remain constant as shown in \cite{Agrawal2004}. If a mechanism's configuration can be completely by a vector of joint values \(\boldsymbol{\theta}\), then we define the potential energy of the mechanism due to gravity to be \(V_m(\boldsymbol{\theta})\).  Letting $V_e(\boldsymbol{\theta})$ be the total elastic energy in the system, the total energy, \(V(\boldsymbol{\theta})\), is:

\begin{equation}
V(\boldsymbol{\theta})=V_m(\boldsymbol{\theta})+V_e(\boldsymbol{\theta})
\end{equation}

\noindent
which dictates that the following relation for the elastic potential in the mechanism must hold true:

\begin{equation}
\frac{\partial V_e(\boldsymbol{\theta})}{\partial \boldsymbol{\theta}}=-\frac{\partial V_m(\boldsymbol{\theta})}{\partial \boldsymbol{\theta}}
\end{equation}

The proposed method for balancing the mechanism is to use wire rope connected to linear springs and attached to various links in the structure after passing through non-circular pulleys.  These non wire cams will modulate the elongation of the springs to minimize change in the potential energy of the entire system.  The energy stored in a spring can be written as:

\begin{equation}
V_e\left(\boldsymbol{\theta}\right)=\frac{1}{2}\Delta\mathbf{x}\left(\boldsymbol{\theta}\right)^T\mathbf{K}\Delta\mathbf{x}\left(\boldsymbol{\theta}\right)
\end{equation}

\noindent
where $\Delta\mathbf{x}$ is the elongation of the spring from its natural length and $\mathbf{K}$ is a positive definite stiffness matrix.

In the following subsections, the kinematics of a serial and parallel mechanism chain will be defined and a generalized potential function presented.  These potential functions will then be used to design the cam profiles to achieve balancing.

%\subsection{Serial Mechanisms}
%The type of serial mechanism discussed in this paper is a series of rigid links connected by actuated revolute joints.  Prismatic joints will be discussed in the next section although they could easily be added into a serial kinematic chain.  For the \(i'th\) rigid link, the vector  $^{i}\mathbf{a}_i$ specifies the location of the following link's frame and the vector $^{i}\mathbf{c}_i$ defines the center of mass of the \(i'th\) link in its own frame.  The mass of the link is defined by $m_i$. The superscript denoting the vector's frame will be omitted unless it is not being expressed in its local frame. Rotation of the rigid link is about its local $\hat{\mathbf{z}}$ axis. Fixed rotation about the $\hat{\mathbf{z}}$ and $\hat{\mathbf{z}}$ axes may be parameterized by $\alpha_i$ and $\beta_i$ respectively. Figure \ref{fig:serial_mechanism} shows a schematic representation of the serial chain's definition.
%
%\begin{figure}
%\includegraphics[width=1\columnwidth]{figures/PNG/serial_link_vectors.png}
%\caption{A general serial mechanism with revolute links.  For the \(i'th\) link, the vector $\mathbf{c}_i$ specifies the link's center of mass (magnitude of $m_i$) with respect to the local frame. The vector $\mathbf{a}_i$ defines the origin of the $i+1$ link in the \(i'th\) link frame. \label{fig:serial_mechanism}}
%\end{figure}
%
%
%Given a gravity acceleration vector $\hat{\mathbf{g}}$ and homogeneous transformations of frame $i$ in frame $j$ expressed as $^{j}\mathbf{T}_i$; the gravitational potential can be written as:
%
%\begin{equation}
%V_m(\boldsymbol{\theta})=\left(\sum\limits_{i=1}^{N}{m_i}\left[{^{0}\mathbf{T}_i }\mathbf{c}_i+\left(\sum\limits_{j=1}^{i-1} {^{0}\mathbf{T}_j} \mathbf{a}_i\right)\right]\right)\cdot{\hat{\mathbf{g}}}
%\end{equation}
%
%Upon differentiating the potential energy, the terms in each partial derivative may be written as summations of basic trigonometric functions with coefficients based on mass distribution and geometry of the links.  We denote the $i'th$ row and $j'th$ column of matrices $\mathbf{A}$ and $\mathbf{B}$ as $a_{i,j}$ and $b_{i,j}$ and designate them as the potential weight matrices.  The partial derivatives of the potential function are then written as:
%
%\begin{equation}
%\frac{\partial V_m(\boldsymbol{\theta})}{\partial \theta_i}=\sum\limits_{j=i}^{N}\left[a_{i,j}\cos(\sum\limits_{k=1}^{j}\theta_k)+b_{i,j}\sin(\sum\limits_{k=1}^{j}\theta_k)\right]
%\end{equation}
%
%\noindent
%This equation implies that in the general case, this class of serial mechanism could be balanced if the following conditions could be met:
%\begin{enumerate}
%  \item The compensating elastic mechanism can generate arbitrary trigonometric curves.
%  \item A coupling scheme could be employed to capture sequential sums of joint angles (i.e. $\sum\limits_{i=1}^{N}\theta_i$)
%\end{enumerate}
%
%Showing that the first requirement can be met is left to the following section however assuming it is true the rest of this kinematics section addresses the second requirement.  Shown in Fig. \ref{fig:serial_wire_actuation} is a wire routing configuration where wire loops terminating on the rigid links are routed to capstans resulting in coupled actuation of the links at the capstans.  In the figure, capstan rotation angles are $\psi_i$ and joint rotations relative to the previous link as $\theta_i$. The configuration shown follows the relationship:
%
%\begin{equation}
%\psi_i=\sum\limits_{j=1}^{j}\theta_i
%\end{equation}
%
%Tsai \cite{Tsai1999} presented a convenient method of relating the capstan rotation to the joint angle through a structural matrix $S$ for which the relationship $\boldsymbol{\theta}=\mathbf{S}\boldsymbol{\psi}$ holds.  A thorough review of generating this matrix can be found in CITE. When the radii of all idler pulleys and capstan in a wire loop are equal then the structural matrix for the three link chain in Fig. \ref{fig:serial_wire_actuation} is:
%
%\begin{equation}
%\mathbf{S}=
%\left[\begin{matrix}
%1&0&0\\
%-1&1&0\\
%0&-1&1 \end{matrix}\right]
%\end{equation}
%
%
%
%\begin{figure}
%\includegraphics[width=1\columnwidth]{figures/PNG/serial_wire_actuation.png}
%\caption{Wire actuation in a serial revolute link chain. \label{fig:serial_wire_actuation}}
%\end{figure}
%
%
%\subsection{Parallel Mechanisms}




\begin{figure}
\includegraphics[width=1\columnwidth]{figures/PNG/wire_cam_schematic.png}\\
  \caption{Wire cam diagram.}\label{fig:wire_cam_schematic}
\end{figure}

The shape of the cam is defined in a two dimensional polar coordinate system with an angle $\phi$ and a radius $g(\tilde{\phi})$ where $\theta$ is the rotation of the cam and $\tilde{\phi}=\phi-\theta$. Figure \ref{fig:wire_cam_schematic}
provides a schematic representation of a single cam and idler pulley connected by a wire.  The origin is centered on the axis of revolution of the cam.  A point on the cam edge is defined as $\mathbf{c}(\phi)=g(\tilde{\phi})\hat{\mathbf{c}}(\phi)$ where $\hat{\mathbf{c}}(\phi)=\left[\cos(\phi),\sin(\phi),0\right]^T$. The tangent unit vector to a point on the cam is:

\begin{equation}
\hat{\mathbf{t}}=\frac{\frac{d\mathbf{c}}{d\phi}}{\|\frac{d\mathbf{c}}{d\phi}\|}=\frac{\frac{dg}{d\phi}\mathbf{c}+g(\phi)\frac{d\mathbf{c}}{d\phi}}{\sqrt{g(\phi)^2+\left(\frac{dg}{d\phi}\right)^2}}
\end{equation}

\noindent
The normal vector to a point on the cam can them be written as:
\begin{equation}
\hat{\mathbf{n}}=\hat{\mathbf{z}}_0\times\hat{\mathbf{t}}
\end{equation}

\noindent
The wire between the cam and the idler pulley must be tangent to both which leads to the following loop closure equation:

\begin{equation}
\mathbf{d}+\mathbf{e}=\mathbf{c}+\lambda\hat{\mathbf{t}}
\label{eq:loop_closure}
\end{equation}

The vector $\mathbf{e}$, defining the point of tangency on the idler pulley, can be written as:
\begin{equation}
\mathbf{e}=\pm{r}\hat{\mathbf{n}}\label{eq:e_vector}
\end{equation}

\noindent
Substituting \ref{eq:e_vector} into \ref{eq:loop_closure} along with the fact that $\hat{\mathbf{n}}^T\hat{\mathbf{t}}$ and solving for $\lambda$ yields:

\begin{equation}
\lambda=\hat{\mathbf{t}}^T\left(\mathbf{d}-\mathbf{c}\right)
\end{equation}

After obtaining the value of $\lambda$ for a given polar coordinate $\phi$, the next goal is to find the value of $\phi$ which closes the loop.  We denote this solution as $\phi_c$.  There are four possible configurations for the wire configuration as shown in Fig \ref{fig:wire_cam_schematic}.

\begin{equation}
h(\tilde{\phi})=\hat{\mathbf{n}}^T\left(\mathbf{d}-\mathbf{c}-\lambda\hat{\mathbf{t}}\right)\pm r=\hat{\mathbf{n}}^T\left(\mathbf{d}-\mathbf{c}\right)\pm r
\end{equation}

\noindent
Defining the angle of $\mathbf{d}$ as $\gamma=\arctan\left(\frac{d_y}{d_x}\right)$ the wire solution is found in one of the following domains:

\begin{table}
  \centering
  \begin{tabular}{| c | c | c |}
     \hline
     % after \\: \hline or \cline{col1-col2} \cline{col3-col4} ...
     Case & $\phi\in$ & $r$ \\
     \hline
     1 & $\left[\gamma-\pi, \gamma\right]$ & $-r$ \\
     \hline
     2 & $\left[\gamma, \gamma+\pi\right]$ & $-r$ \\
     \hline
     3 & $\left[\gamma-\pi, \gamma\right]$ & $+r$ \\
     \hline
     4 & $\left[\gamma, \gamma+\pi\right]$ & $+r$ \\
     \hline
   \end{tabular}
  \caption{Wire Case Definitions}\label{tab:wire_configurations}
\end{table}

The length $L$ of the wire can be written as:

\begin{equation}
L=\lambda+\pi\left(\beta-\beta_0\right)+\int_{\tilde{\phi}_0}^{\tilde{\phi}_c}\sqrt{g(\phi)^2+\left(\frac{dg(\phi)}{d\phi}\right)^2}d\phi
\end{equation}



%\subsection{Differential Kinematics}
%
%\begin{equation}\label{eq:constraint_deriv}
%\frac{dh}{dg}\frac{dg}{d\tilde{\phi}}\frac{d\tilde{\phi}}{d\phi}\dot{\phi}+\frac{dh}{d\phi}\dot{\phi}+\frac{dh}{dg}\frac{dg}{d\tilde{\phi}}\frac{d\tilde{\phi}}{d\theta}\dot{\theta}=0
%\end{equation}
%
%\noindent
%Given that $\frac{d\tilde{\phi}}{d\phi}=1$ and $\frac{d\tilde{\phi}}{d\theta}=-1$:
%
%\begin{equation}
%\left(\frac{dh}{dg}\frac{dg}{d\tilde{\phi}}+\frac{dh}{d\phi}\right)\dot{\phi}=\frac{dh}{dg}\frac{dg}{d\tilde{\phi}}\dot{\theta}
%\end{equation}
%
%\begin{equation}
%\dot{\phi}=\left(\frac{\left. \frac{dh}{d\tilde{\phi}}\right|_{\phi_c,\theta}}{\left.\frac{dh}{d\tilde{\phi}}\right|_{\phi_c,\theta}+\left.\frac{dh}{d\phi}\right|_{\phi_c,\theta}}\right)\dot{\theta}
%\end{equation}
%
%\begin{equation}
%\left(\frac{dh}{dg}\frac{dg}{d\tilde{\phi}}+\frac{dh}{d\phi}\right)\dot{\phi}=-\frac{dh}{dg}\frac{dg}{d\alpha_i}\dot{\alpha}_i
%\end{equation}
%
%\begin{equation}
%\dot{\phi}=\left(\frac{\left. \frac{dh}{d\alpha_i}\right|_{\phi_c,\theta}}{\left.\frac{dh}{d\tilde{\phi}}\right|_{\phi_c,\theta}+\left.\frac{dh}{d\phi}\right|_{\phi_c,\theta}}\right)\dot{\alpha}_i
%\end{equation}







